Incremental Image Labeling via Iterative Refinement

Data quality is critical for multimedia tasks, while various types of systematic flaws are found in image benchmark datasets, as discussed in recent work. In particular, the existence of the semantic gap problem leads to a many-to-many mapping between the information extracted from an image and its linguistic description. This unavoidable bias further leads to poor performance on current computer vision tasks. To address this issue, we introduce a Knowledge Representation (KR)-based methodology to provide guidelines driving the labeling process, thereby indirectly introducing intended semantics in ML models. Specifically, an iterative refinement-based annotation method is proposed to optimize data labeling by organizing objects in a classification hierarchy according to their visual properties, ensuring that they are aligned with their linguistic descriptions. Preliminary results verify the effectiveness of the proposed method.

==> Algorithms/algorithm1.tex <==

\begin{algorithm}[!t] \small
\caption{OracleRC Annotation Process in Radical and Structure Level. \\
$R_L, R_C, S_L  = LabelRaS(I)$}
% x_1, y_1, x_2, y_2
\label{alg:1}
\begin{algorithmic}[1]
\Require Oracle images $I$, Oracle KG $ZiNet$
\Ensure Labels of radicals in Oracle images $R_L$, radical localization coordinates $R_C$, and structural relation-label $S_L$.
% $x_1$, $y_1$, $x_2$, and $y_2$, 

\State $n = getRadicalNumber(I, $ZiNet$)$;
\If {$n = 1$}\label{algln2}
    \State $R_L = C_L$;
    \State $R_c = getCoordinates(I, M_{OL})$;
    % \{Get radical localization coordinates $R_C$ with the trained model $M_{OL}$.\}
    \State $S_L = Single$;
    % \{The structure-level label $S_L$ is $Single$.\}
\Else
        \While {$R_i \in C(I)$}
        \State $R_{Li1}, R_{Ci1} = ELR_{G1}(I)$;   
        \State $R_{Li2}, R_{Ci2} = ELR_{G2}(I)$;
        % \{Two experts belonging to two groups $G1$ and $G2$ annotate the $i_{th}$ radicals in the character image with labels and localization coordinates, respectively. \}
        \If {$R_{Li1} = R_{Li2}$}
            \State $R_{Li} = R_{Li1}$;
        \Else
            \State $R_{Li}, R_{Ci} = SELR_{G3}(I)$;  
            % \{If the results of the radical category annotations of the two experts are inconsistent, a senior expert, will re-annotate and determine the final annotation of the radical category and localization coordinates. \}
        \EndIf 
        \State $R_L.add(R_{Li})$;
        \State $R_C.add(R_{Ci})$;
        \EndWhile
    \State $S_{L1} = ELS_{G1}(I)$;
    \State $S_{L2} = ELS_{G2}(I)$;
    \If {$S_{L1} = S_{L2}$}
        \State $S_{L} = S_{L1}$;
    \Else
        \State $S_{L} = SELS_{G3}(I)$;
    \EndIf
\EndIf \\
\Return $R_{L}, R_{Ci}, S_{L}$; 
\end{algorithmic}
\end{algorithm}



% \State Collecting oracle images $I$ and corresponding character-labels $C_L$ from book $B$. 
% \State Applying denoising method for every oracle image $I$. 
% \State Cleaning $I$, including deleting images not oracle characters and unrecognizable characters with too much noise. 
% \State Annotating radicals in $I$ with LabelImg tool, and getting radical-label $R_L$, structural relation-label $S_L$ and radical localization $x_1$, $y_1$, $x_2$, and $y_2$.  
% \State Proofreading annotation results, and geting the final labels including $C_L$, $R_L$, $S_L$ $x_1$, $y_1$, $x_2$, and $y_2$. 

==> Algorithms/algorithm2.tex <==
\begin{algorithm}[!t] \small
\caption{Splicing-based synthetic character image generation. 
$Set_{syn}  = GenImg(Set_{R}, Set_{S})$}
% x_1, y_1, x_2, y_2
\label{alg:2}
\begin{algorithmic}[1]
\Require Radical image set $Set_{R}$, character structure set $Set_{S}$.
\Ensure Synthetic character image set $Set_{syn}$.



\While {$str \in Set_{S}$}
    \State $S_L = str$;
    \State $Num_R, Loc_R = getStructure(str)$;   

    \While {$j \in range(n)$}
        
    \State $List_{tem} = getRadicals(Set_R, Num_R)$;
    \State $List_R = augmentImg(List_{tem})$;
        
    \State $R_L, R_C = getInfo(List_R)$;
    \State $I_{syn} = generateImg(List_R, Loc_R)$;
    \State $Syn_j.append(\{I_{syn}, R_L, R_C, S_L\})$
    % \State $I_{syn} = finetuneImg(I_{temp})$
    % 是否需要加上一个用判断器判断其是否是oracle的步骤？     
\EndWhile
    \State $Set_{syn}.append(Syn_j)$;
\EndWhile \\
\Return $Set_{syn}$; 
\end{algorithmic}
\end{algorithm}
